Compactified Spacelike Extra Dimension & Brane-Higgs Field

In the paradigm with a small warped Spacelike Extra Dimensions (SED), the Higgs field is in general localized at a boundary of the SED (TeV-brane) where the gravity scale is redshifted to the TeV by a warp factor. If the SM gauge bosons and fermions propagate into the warped SED, one can generate the mass hierarchy for fermions. It is thus crucial to treat carefully the TeV-brane localized masses for such fermions, which is done in the literature by applying a regularization process suffering from a lack of consistency and more importantly being useless, as we demonstrate in detail in the present thesis. The first part of the thesis is devoted to the treatment of brane localized mass terms for 5D fermions, which requires the introduction of new Lagrangian terms at the SED boundaries, similar to the Gibbons-Hawking terms in gravity. The second part consists in applying different methods (function/distribution fields, 4D/5D calculations, etc) to various brane localized terms (kinetic terms, Majorana masses, etc), as well as a generalization to several classified models (flat/warped dimensions, intervalle/orbifold, etc). In the third part, we propose to compactify a flat SED on a star/rose graph with a large number of identical small leaves/petals. We obtain a compactified space with a large volume without a large compactification length to stabilize. We use the approach of 5D fermions to build a toy model of small Dirac neutrino masses (brane localized left-handed neutrinos and bulk right-handed ones).

==> annexe4.tex <==
% Alternative Method for the Orbifold $S^1/\mathbb{Z}_2
In this appendix, we present an alternative treatment of the model of Subsection~\ref{1_Orbifold} with an extra dimension compactified on the orbifold $S^1/\mathbb{Z}_2$, where we do not use distribution theory.

The action is
\begin{align}
S_{Fermion} = S_{\Psi} + S_{Y} + S_B \, ,
\label{a_S_Psi_S1/Z2_Lagrangian}
\end{align}
with $S_{\Psi}$,  $S_{Y}$ and $S_B$ defined as the actions of the kinetic terms, the brane localized Yukawa interactions and the BBTs respectively ($L = \pi R$):
\begin{align}
&S_{\Psi} = \int d^4x \int_{-L^+}^{L} dy \ \mathcal{L}_\Psi \, , 
\label{a_1_eq:actionKin}
\end{align}
with $\mathcal{L}_\Psi$ defined in Eq.~\eqref{1_L_2},
\begin{align}
&S_{Y} = \int d^4x  \ \mathcal{L}_Y |_{L} \, , 
\label{a_1_eq:actionYuk}
\end{align}
with $\mathcal{L}_Y$ defined in Eq.~\eqref{a_1_eq:actionYuk}, and
\begin{align}
S_B  &=  \int d^4x \  \dfrac{1}{2} \left[ \left. \left( \bar{D}D - \bar{Q}Q \right) \right |_{-L^+}^{0^-} + \left. \left( \bar{D}D - \bar{Q}Q \right)\right |_{0^+}^{ L^-}  \right]  \, .
\label{a_1_eq:actionBound}
\end{align}

When calculating the mass spectrum of the KK fermions, we restrict our attention to the VEV $v$ of $H$ \eqref{1_H_exp}. Hence, we decompose the Yukawa interactions into $S_Y = S_X + S_{hQD}$ and the action involving only the fermions becomes:
\begin{align}
S_{Fermion}^{X} = S_{\Psi} + S_{X} + S_B \, .
\label{a_S_Psi_S1/Z2_Lagrangian_VEV}
\end{align}
\begin{align}
&S_{X} = \int d^4x \ \mathcal{L}_X |_{L} , \nonumber \\
&\text{with} \ \ 
\mathcal{L}_X = - X\ Q^\dagger_L D_R - X^\prime\ Q^\dagger_RD_L +  {\rm H.c.} \ ,
\label{a_1_L_5}
\end{align}
with the compact notations $X = \dfrac{v}{\sqrt{2}} \, Y_5$, $X' = \dfrac{v}{\sqrt{2}} \, Y_5'$, and
\begin{align}
&S_{hQD} = \int d^4x \ \mathcal{L}_{hQD} |_{L}  \ , \nonumber \\
&\text{with} \ \ 
\mathcal{L}_{hQD} = - \dfrac{Y_5}{\sqrt{2}} \ h Q^\dagger_L D_R - \dfrac{Y_5'}{\sqrt{2}} \ h Q^\dagger_RD_L +  {\rm H.c.} \ .
\label{a_1_L_Yuk}
\end{align}

We begin by cutting the integral over $y$ of the kinetic terms \eqref{a_S_Psi_S1/Z2_Lagrangian_VEV} at the brane-Higgs position:
\begin{align}
S_{\Psi} &= \int d^4x \int_{-L^+}^{L} dy \ \mathcal{L}_\Psi  \nonumber \\
&= \int d^4x \ \left \{  \int_{-L^+}^{0^-} dy \ \mathcal{L}_\Psi + \int_{0^+}^{L^-} dy \ \mathcal{L}_\Psi \right \} \, ,
\label{a_1_eq:actionKin_cut}
\end{align}
where the partial derivatives with respect to $y$ of the 5D fields are defined on the right side of $y=L$. The 5D fields are thus continuous on the right side of $y=L$.

We choose the transformation laws for the fermionic fields $Q$ and $D$ under $\mathbb{Z}_2$ as:
\begin{equation} 
\left\{
\begin{array}{c c c}
Q \left( x^\mu, -y \right) = - \gamma^5 \, Q \left( x^\mu, y \right) \, \Longrightarrow \, Q_L \ \text{even}, \ Q_R \ \text{odd},
\\ \vspace{-0.2cm} \\
D \left( x^\mu, -y \right) = \gamma^5 \, D \left( x^\mu, y \right) \, \Longrightarrow \, D_L \ \text{odd}, \ D_R \ \text{even}.
\end{array}
\right.
\label{a_1_Z2}
\end{equation}

Considering the Lagrangian symmetry $\mathbb{Z}_2$, and performing a change of variable in the kinetic terms \eqref{a_1_eq:actionKin_cut}:
\begin{align}
S_{\Psi} &\ni \int d^4x \ \int_{-L^+}^{0^-} dy \ \mathcal{L}_\Psi  \nonumber \\
&= \int d^4x \ \int_{0^+}^{L^-} dy' \ \mathcal{L}_\Psi \nonumber \\
&= \int d^4x \ \int_{0^+}^{L^-} dy \ \mathcal{L}_\Psi \ , \nonumber \\
&\text{with $y'=y+L$.}
\label{a_1_eq:actionKin_cut_Label}
\end{align}

Then we separate the brane localized mass terms into two identical parts by the continuity of the 5D fields on the left side of $y=L$ and we use the symmetry under $\mathbb{Z}_2$:
\begin{align}
S_{X} &= \int d^4x \ \mathcal{L}_X |_{L} = \int d^4x \ \mathcal{L}_X |_{L^-}  \nonumber \\
&= \int d^4x \ \dfrac{1}{2} \left[  \mathcal{L}_X |_{L^-} + \mathcal{L}_X |_{-L^+} \right]  \ , \nonumber \\
&\text{where $\mathcal{L}_X |_{L^-} = \mathcal{L}_X |_{-L^+}$. }
\label{a_1_L_5_2}
\end{align}

We can also use the transformation laws \eqref{a_1_Z2} in the BBTs \eqref{a_1_eq:actionBound}:
\begin{align}
S_B & \ni  \int d^4x \  \dfrac{1}{2} \left. \left( \bar{D}D - \bar{Q}Q \right) \right |_{-L^+}^{0^-} \nonumber \\
&= \int d^4x \  \dfrac{1}{2} \left\{ \left. \left( D^ \dagger \gamma^5 \gamma^0  \gamma^5 D - Q^ \dagger \gamma^5 \gamma^0  \gamma^5 Q \right) \right |_{L^-}^{0^+} \right\} \nonumber \\
&= \int d^4x \  \dfrac{1}{2} \left. \left( \bar{D}D - \bar{Q}Q \right) \right |_{0^+}^{L^-} \ .
\label{a_1_eq:actionBound_s}
\end{align}

We rewrite $S_{Fermion}^{X}$ as
\begin{align}
S_{Fermion}^{X} &= S_{\Psi} + S_{X} + S_B \nonumber \\
&= \int d^4x  \left \{  \int_{-L^+}^{0^-} dy \ \mathcal{L}_\Psi + \int_{0^+}^{L^-} dy \ \mathcal{L}_\Psi \right \} 
+ \int d^4x \ \dfrac{1}{2} \left[  \mathcal{L}_X |_{L^-} + \mathcal{L}_X |_{-L^+} \right] \nonumber \\
&+  \int d^4x \  \dfrac{1}{2} \left[ \left. \left( \bar{D}D - \bar{Q}Q \right) \right |_{-L^+}^{0^-} + \left. \left( \bar{D}D - \bar{Q}Q \right)\right |_{0^+}^{ L^-}  \right] \nonumber \\
&= \int d^4x \ \left[  \int_{-L^+}^{0^-} dy \ \mathcal{L}_\Psi + \left. \dfrac{1}{2} \mathcal{L}_X \right |_{-L^+} + \left. \dfrac{1}{2} \left( \bar{D}D - \bar{Q}Q \right) \right |_{-L^+}^{0^-} \right] \nonumber \\
&+ \int d^4x \ \left[ \int_{0^+}^{L^-} dy \ \mathcal{L}_\Psi + \left. \dfrac{1}{2} \mathcal{L}_X \right |_{L^-} + \left. \dfrac{1}{2} \left( \bar{D}D - \bar{Q}Q \right)\right |_{0^+}^{ L^-}  \right]  \nonumber \\
&= S_{Fermion 1}^{X} + S_{Fermion 2}^{X} \ ,\nonumber\\
\text{with} \ \ 
S_{Fermion 1}^{X} &=\int d^4x \ \left[  \int_{-L^+}^{0^-} dy \ \mathcal{L}_\Psi + \left. \dfrac{1}{2} \mathcal{L}_X \right |_{-L^+} + \left. \dfrac{1}{2} \left( \bar{D}D - \bar{Q}Q \right) \right |_{-L^+}^{0^-} \right] \ , \nonumber \\
S_{Fermion 2}^{X} &=\int d^4x \ \left[ \int_{0^+}^{L^-} dy \ \mathcal{L}_\Psi + \left. \dfrac{1}{2} \mathcal{L}_X \right |_{L^-} + \left. \dfrac{1}{2} \left( \bar{D}D - \bar{Q}Q \right)\right |_{0^+}^{ L^-}  \right]  \ .
\label{a_SF_Z2_1&2}
\end{align}

Using \eqref{a_1_eq:actionKin_cut_Label}, \eqref{a_1_L_5_2}, \eqref{a_1_eq:actionBound_s} into \eqref{a_SF_Z2_1&2}, we find the identity:
\begin{align}
S_{Fermion 1}^{X} =S_{Fermion 2}^{X}  \ .
\label{a_SF_1&2}
\end{align}

Finally, we separate the action $S_{Fermion}^{X}$ \eqref{a_S_Psi_S1/Z2_Lagrangian_VEV} into 2 identical parts:
\begin{align}
S_{Fermion}^{X} =2 \ S_{Fermion 2}^{X}  \ .
\label{a_SF_tot}
\end{align}
We can thus treat $S_{Fermion 2}^{X}$ as the basic building block and go back to the interval scenario $[0, L]$ in Subsection~\ref{1_Correct_treatment_AFHS_term}. If we search for the profiles in $(-L, 0)$, we just need to use the transformation laws \eqref{a_1_Z2} for fermionic fields $Q$ and $D$.
\begin{table}[h]
\centering
\begin{tabular}{| c | c | c | c | c | }
\hline
\multirow{2}{*}{\diagbox{Domains}{Fields}} & \multicolumn{2}{| c |}{$Q_{L/R}$} & \multicolumn{2}{| c |}{$D_{L/R}$}  \\
\cline{2-5}
 & $q^n_L(y)$ & $q^n_R(y)$ & $d^n_L(y)$ & $d^n_R(y)$ \\
\hline
$(-L, 0)$ & $A^n_{q} \; \cos(M_n \; y)$ & $A^n_{q} \; \sin(M_n \; y)$ & $- A^n_{d} \; \sin(M_n \; y)$ & $A^n_{d} \; \cos(M_n \; y)$  \\
\hline
$[0, L]$ & $A^n_{q} \; \cos(M_n \; y)$ & $A^n_{q} \; \sin(M_n \; y)$ & $- A^n_{d} \; \sin(M_n \; y)$ & $A^n_{d} \; \cos(M_n \; y)$ \\
\hline
Mass spectrum & \multicolumn{4}{| c |}{$M_n = \dfrac{1}{L} \left[ n \pi + \arctan \left( \dfrac{|X|}{2} \right) \right] \, , n \in \mathbb{Z}$}  \\
\hline
\end{tabular}
\caption{Fermionic fields Q and D on the flat orbifold $S^1/ \mathbb{Z}_2$.}
\label{a_Q&D_Z2}
\end{table}


